A Weak Supervision Approach to Detecting Visual Anomalies for Automated Testing of Graphics Units

We present a deep learning system for testing graphics units by detecting novel visual corruptions in videos. Unlike previous work in which manual tagging was required to collect labeled training data, our weak supervision method is fully automatic and needs no human labelling. This is achieved by reproducing driver bugs that increase the probability of generating corruptions, and by making use of ideas and methods from the Multiple Instance Learning (MIL) setting. In our experiments, we significantly outperform unsupervised methods such as GAN-based models and discover novel corruptions undetected by baselines, while adhering to strict requirements on accuracy and efficiency of our real-time system.

==> previouswork.tex <==
The weak supervision approach in this paper is an enhancement we developed to our system \cite{Faivishevsky2018AutomatedTO}. Our visual corruption detection system captures the display using a camera (screen grabbing does not enable testing the actual displays used). The captured videos are then analyzed using deep neural network models. In our previous work, labeled data was collected with manual tagging. As real cases of corruption (Figure \ref{fig:SystemAndCorruptionExamples}) were relatively rare, we collected corrupted examples by reproducing past bugs. For more details about this collection process, see \cite{Faivishevsky2018AutomatedTO}.

%We also captured a large amount, about 15 hours, of diverse good uncorrupted data to ensure high variability of the content in the dataset.

Our main focus in \cite{Faivishevsky2018AutomatedTO} was supervised learning with Deep CNN topologies to obtain high accuracy on known corruptions. We additionally applied unsupervised methods to try and capture novel corruptions and reduce manual tagging.

%Rather than using purely unsupervised models, in this work we explore weak supervision to benefit from the generalization and scalability afforded by unsupervised learning, but also improve accuracy. 
